What to Read in a Contract? Party-Specific Summarization of Legal Obligations, Entitlements, and Prohibitions

Reviewing and comprehending key obligations, entitlements, and prohibitions in legal contracts can be a tedious task due to their length and domain-specificity. Furthermore, the key rights and duties requiring review vary for each contracting party. In this work, we propose a new task of party-specific extractive summarization for legal contracts to facilitate faster reviewing and improved comprehension of rights and duties. To facilitate this, we curate a dataset comprising of party-specific pairwise importance comparisons annotated by legal experts, covering ~293K sentence pairs that include obligations, entitlements, and prohibitions extracted from lease agreements. Using this dataset, we train a pairwise importance ranker and propose a pipeline-based extractive summarization system that generates a party-specific contract summary. We establish the need for incorporating domain-specific notion of importance during summarization by comparing our system against various baselines using both automatic and human evaluation methods

==> sections/aahuman_eval.tex <==
\section{Human Evaluation of Summaries} \label{sec:human-eval}
In addition to automatic evaluation, we also give contracts along with their \textit{party-specific} summaries from \textsc{ContraSum}, gold-references (CR=$0.15$), the best baseline-LexRank (PC), and Random (PC) baseline to legal experts for human evaluation.
$16$ summaries, each consisting of a maximum of $10$ sentences per category, for $2$ contracts are provided to $2$ experts.
They are asked to rate the summaries for each category on a $5$-point scale ($1$ least; $5$ most) as per several criteria: \begin{inparaenum}[(1)]
   \item{informativeness; }
   \item{usefulness;}
   \item{accuracy of categorization;}
   \item{redundancy, and}
   \item{accuracy of importance ranking.}
\end{inparaenum}
In addition, we ask them to rate the overall quality of a summary on a 10-point scale. The average scores are presented in Table~\ref{tab:human}. \textsc{ContraSum} produces the best summaries overall but lacks in the diversity of sentences within each category. Interestingly, experts found summaries from \textsc{ContraSum} to be more informative, useful, and correctly categorized than the gold-references. This may be due to the more number of sentences in the predicted summaries (capped at $10$) than the gold-references (especially for  prohibitions which can be $<$$10$ at CR=$0.15$ for a party). We observed that the experts also considered the importance of a category expressed in a sentence with respect to a party. Hence, they penalize for the accuracy of categorization if the category is indirectly expressed in a sentence for a party (see \ref{subsec:human-eval} for an example and category-wise evaluation results). 
\begin{table}[t!]
\centering
\small
\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Model}&\textbf{Info.}$\uparrow$&\textbf{Use}$\uparrow$&\textbf{AoC}$\uparrow$&\textbf{Red.}$\downarrow$&\textbf{AoIR}$\uparrow$&\textbf{O}$\uparrow$\\
\midrule
Rand&$2.96$& $2.87$& $2.92$&$1.92$&$2.50$&$2.94$\\
LR &$3.00$&$2.79$&$3.04$&$2.04$&$2.46$&$3.06$\\
\textsc{CS}&$\mathbf{3.25}$&$\mathbf{3.37}$&$\mathbf{3.25}$&$2.04$&$2.54$&$\mathbf{3.50}$\\
Ref&$3.17$&$3.00$&$3.17$&$\mathbf{1.75}$&$\mathbf{2.87}$&$3.06$\\
\bottomrule
\end{tabular} 
}
\caption{Results for human evaluation of model summaries. Mean scores of the $2$ annotators are averaged across categories and parties. Overall (O) rating is scaled down to half to make it comparable. Info., Use, AoC, Red., AoIR denote informativeness, usefulness, accuracy of categorization, redundancy, and accuracy of importance ranking, resp. Rand: Random (PC), LR: LexRank (PC), CS: \textsc{ContraSum}, Ref: References. }\label{tab:human}
\end{table}

==> sections/discussion.tex <==
\section{Discussion}
\paragraph{Extending annotation framework to multi-party agreements.} While we demonstrate the annotation process and the proposed summarizer for two-party agreement, our annotation framework could be extended to more complex legal agreements involving multiple parties by taking into consideration each pair of contracting parties. As one party can have obligations towards any of the other parties, Best-worst scaling could be done per pair of parties. For \it {e.g.,} the annotation task could be defined to find the most and least important obligation of Party A towards party B. Similarly from modeling perspective, both parties could be specified in the input.
\paragraph{}
